Fair Near Neighbor Search: Independent Range Sampling in High Dimensions

Similarity search is a fundamental algorithmic primitive, widely used in many computer science disciplines. There are several variants of the similarity search problem, and one of the most relevant is the $r$-near neighbor ($r$-NN) problem: given a radius $r>0$ and a set of points $S$, construct a data structure that, for any given query point $q$, returns a point $p$ within distance at most $r$ from $q$. In this paper, we study the $r$-NN problem in the light of fairness. We consider fairness in the sense of equal opportunity: all points that are within distance $r$ from the query should have the same probability to be returned. In the low-dimensional case, this problem was first studied by Hu, Qiao, and Tao (PODS 2014). Locality sensitive hashing (LSH), the theoretically strongest approach to similarity search in high dimensions, does not provide such a fairness guarantee. To address this, we propose efficient data structures for $r$-NN where all points in $S$ that are near $q$ have the same probability to be selected and returned by the query. Specifically, we first propose a black-box approach that, given any LSH scheme, constructs a data structure for uniformly sampling points in the neighborhood of a query. Then, we develop a data structure for fair similarity search under inner product that requires nearly-linear space and exploits locality sensitive filters. The paper concludes with an experimental evaluation that highlights (un)fairness in a recommendation setting on real-world datasets and discusses the inherent unfairness introduced by solving other variants of the problem.

==> app.tex <==
\subsection{Estimating nearborhood size}\label{sec:sampling_bias}
Let $\hat B_S(q,r)$  be the set of points in $B_S(q,r)$ that collides at least one with a query point $q$, and let $\hat b_S(q,r)=\cup B_S(q,r)$. 
Let also $C(q,r)$
The value of $\hat b_S(q,r)$ can be simply computed by scanning the $L$ buckets where $q$ collides and counting the number of $r$-near points.
However, such approach requires $\BTO{b_S(q,r)p_1^{-1}+b_S(q,c\cdot r)}$.
We show how such a value can be efficiently estimated in a two step approach: we first estimate the number $c_S(q)$ of distinct points colliding with $q$ (the points can be $r$-near, $cr$-near, or far); then by sampling, we estimate how many of the colliding points are actually $r$-near.

The number $c_S(q)$ of colliding points cannot be computed by just summing the size of the buckets where the query $q$ collides: 
indeed, there can be points that collide several times with $q$.
We thus leverage on the sketch for counting distinct elements in \cite{BarYossefJKST02}, that we have recalled in Section \ref{sec:sketch}.
If we use $L$ LSH functions, we then add to each bucket in $S_{i,j}$ the sketch obtained with points in $S_{i,j}$.
Then, at the query time, we take the $L$ sketches of the bucket where $q$ collides, and we merge them. 
The final sketch then gives an $\epsilon$-approximation $\tilde c_S(q)$  of $c_S(q)$  with probability at least $1-\delta$.

For the second part we leverage on the sampling approach with repetition in Section \ref{}.
By sampling $T={}$ points, we can get an $\epsilon$-approximation $\tilde \rho_q$ of the ratio $\rho(q) = b_S(q,r)/c_S(q)$ with probability at least $1-\delta$.
By computing $\tilde \rho_q \cdot \tilde c_S(q)$ we get an $\epsilon$ approximation of $b_S(q,r)$ with probability at least $1-\delta$.

We thus have the following theorem.
\begin{theorem}
For any given query $q$, the above algorithms gives an $\epsilon$-approximation of  $b_S(q,r)$ with probability at least $1-\delta$. 
\end{theorem}



\subsection{Discrimination Discovery}\label{sec:discrimination}

\subsection{Privacy preserving}\label{sec:sampling_privacy}


==> maximization.tex <==
\subsection{Efficiently computing a diverse neighborhood}
\subsection{Computing a fair and diverse neighborhood} 

==> nnwis.tex <==
This section describes how our data structure can handle the weighted case. Let 
$U = [0, u)$ denote the universe of weights. Each point $\p$ in $S$ is 
associated with a weight $w(\p) \in U$.
For a set $B$, will use the notation $w(B) = \sum_{\p \in B} w(\p)$ to denote the 
sum of weights of all points in the set $B$.

The goal when answering query $\q$ is to report each point $\p \in B_S(\q, r)$ with probability roughly equal
to $w(\p)/w(B_S(\q, r))$.  

\paragraph{Construction} Split $S$ up into $S_1, \ldots, S_{\log u}$ 
such that $S_i = \{\p \in S \mid w(\p) \in [2^{i - 1}, 2^i)\}$. 
Next, build data structure $\text{DS}_i$ described in Section~\ref{sec:independent:sampling} for $S_i$. 


\paragraph{Query} On query $\q$, obtain estimates $\hat{n}_1, \ldots, \hat{n}_{\log u}$ from the HLL
counters. Define $W = \sum_{1 \leq i \leq \log u} \hat{n}_j 2^j$.
Choose a random index $i \in \{1,\ldots, \log u\}$ such that $i$ is $j$ with probability $\frac{\hat{n}_j 2^j}{W}$. 
Run the query algorithm described in Section~\ref{sec:independent:sampling} on $\text{DS}_i$ and return its answer. 
%With probability $w(\p) / 2^i$, declare success and return $\p$, otherwise repeat the query on $\text{DS}_i$.

\begin{theorem}
The algorithm described above solves the $r$-near neighbor weighted independent sampling problem and has expected running time $O(n^\rho \log^2 n)$ for $u \leq ???$.
\end{theorem}

\begin{proof}
Fix $\q$ and let $\p$ be a point in $B_S()\q,r)$. 
We have to show that $\p$ is returned with probability $w(\p)/w(B_S(\q, r))$. 
For $\p$ to be returned, the query algorithm has to pick the correct level $i$ and return $\p$ on this level. 
Using Lemma~\ref{lem:independent}, we know that $\p$ is a random point among all the points in $B_S(\q, r)$ that have weight in $[2^{i - 1}, 2^i)$. 
Thus, we may compute the probability that $\p$ is returned as
\begin{align*}
\frac{\hat{n}_i 2^i}{\sum_{j = 1}^{\log u}\hat{n}_j 2^j} \cdot \frac{1}{|S_{\q, i}|}.
\end{align*}
Since $1 \leq \hat{n}_i/|S_{\q, i}| \leq 4$ and $w(B_S(\q, r))/ 2 \leq \sum_{j = 1}^{\log u} \hat{n}_j2^j \leq 8 w(B_S(\q, r))$, $\p$ is returned with probability roughly $w(\p)/w(B_S(\q, r))$. \textbf{MAKE MORE PRECISE.}
\end{proof}

\textbf{ALSO POSSIBLE: Repeat $\p$ with probability $w(\p)/2^i$, otherwise repeat. Brings the $w(\p)$ into place, but still only some approximation.}




==> sampling.tex <==
%!TEX root = main.tex

Suppose we have $S_1,\dots,S_t \subseteq U$ and a fully random hash function $h: U \rightarrow [0,1)$.
For a string $s \in \{0,1\}^*$ define the interval $I_s$ consisting of those real numbers in $[0,1)$ whose binary encoding starts with $0.s$.
Let $n_i = |S_i|$.
Then we organize $S_i$ in buckets indexed by $s\in \{0,1\}^{\lceil \log (n_i+1)\rceil}$, such that bucket $s$ contains $S_i \cap I_s$ (in arbitrary order) and the size $|S_i \cap I_s|$.
Observe that with this organization we can retrieve, for any $s \in \{0,1\}^*$, the elements of $S_i \cap I_s$ in expected time $O(1+|S_i \cap I_s|)$.
(((Give details)))
%If $|s| \leq \lceil \log (n_i+1)\rceil$ this is obvious because 
%This is because the expected number of items per bucket is constant, so even if 

To produce an independent sample from $S = \cup_i S_i$, with failure probability $\delta$, we do the following.
\begin{enumerate}
\item Compute an estimate $\hat{n}$ such that $\hat{n}$ is a power of 2 and $|S|\leq \hat{n} \leq 4\, |S|$ with probability $1-\delta/2$, for example using HyperLogLog counters.
\item Let $b(\hat{n}) = O(\log \hat{n})$ be such that with probability $1-\delta/2$ we have for every $s\in \{0,1\}^{\log \hat{n}}$, $|S\cap I_s| \leq b(\hat{n})$. 
\item Repeat the following until successful:
\begin{enumerate}
	\item Choose $s \in \{0,1\}^{\log{\hat{n}}}$ uniformly at random.
	\item Compute the size $k = |S \cap I_s|$ in expected time $O(t)$.
	\item If $k>b$ declare error and stop.
	\item Otherwise declare success with probability $k/b$; if not succesful go back to step a).
\end{enumerate}
\item Return an element sampled uniformly at random from $S \cap I_s$.
\end{enumerate}

(((Add analysis)))

